Bregman Alternating Direction Method of Multipliers

The mirror descent algorithm (MDA) generalizes gradient descent by using a Bregman divergence to replace squared Euclidean distance. In this paper, we similarly generalize the alternating direction method of multipliers (ADMM) to Bregman ADMM (BADMM), which allows the choice of different Bregman divergences to exploit the structure of problems. BADMM provides a unified framework for ADMM and its variants, including generalized ADMM, inexact ADMM and Bethe ADMM. We establish the global convergence and the $O(1/T)$ iteration complexity for BADMM. In some cases, BADMM can be faster than ADMM by a factor of $O(n/\log(n))$. In solving the linear program of mass transportation problem, BADMM leads to massive parallelism and can easily run on GPU. BADMM is several times faster than highly optimized commercial software Gurobi.

==> cvg_badmm.tex <==
%In optimization, an equality-constrained convex optimization problem is equivalent to solving an unconstrained convex optimization through Lagrangian relaxation.

%In this section, we first discuss the assumptions required in the convergence analysis of BADMM. Then we establish the global convergence for BADMM. Finally, we establish the $O(1/T)$ iteration complexity for BADMM.

%\subsection{Assumptions}
We need the following assumption in establishing the convergence of BADMM:
\begin{asm}\label{asm:badmm}
%\quad
%
(a) $f:\R^{n_1}\!\!\rightarrow\!\!\R\!\cup\!\{+\infty\}$ and $g:\R^{n_2}\!\!\rightarrow\!\!\R\!\cup\!\{+\infty\}$ are closed, proper and convex. %\footnote{$f$ is assumed to be relatively differentiable~\cite{teda12:gbregman} when we define a generalized Bregman divegence $B_f$ in Case 1 of Scenario 2 in Section 2. }.

(b) An optimal solution exists.

(c) The Bregman divergence $B_{\phi}$ is defined on an $\alpha$-strongly convex function $\phi$ with respect to a $p$-norm $\|\cdot\|_p^2$, i.e., $B_{\phi}(\u,\v) \geq \frac{\alpha}{2} \|\u - \v\|_p^2$, where $\alpha > 0$.
%(d) The Bregman divegences $B_{\varphi_\x}(\u,\v) \geq 0, B_{\varphi_\z}(\u,\v) \geq 0$ in Scenario 2.
%(c)  $\y_0 = 0$ and $\| \y \|_2^2 \leq D_{\y}^2, \| \x - \x_0 \|_2 \leq D_{\x}, \| \z - \z_0 \|_2 \leq D_{\z}$. %where $\{\x^*,\z^*,\y^*\}$ is  optimal solution.
%\label{asm:adm1}
\end{asm}

Assume that $\{ \x^*, \z^*,\y^*\}$ satisfies the KKT conditions of the Lagrangian of~\myref{eq:adm_pm} ($\rho = 0$ in~\myref{eq:lag1}), i.e.,
\begin{align}\label{eq:kkt}
-\bA^T\y^* \in \partial f(\x^*)~, -\bB^T\y^* \in \partial g(\z^*)~, \bA\x^* + \bB\z^* - \c = 0~. 
\end{align}
\iffalse
\begin{align}
-\bA^T\y^* & \in \partial f(\x^*)~, \label{eq:kktx}\\
-\bB^T\y^* & \in \partial g(\z^*)~,\label{eq:kktz}\\
\bA\x^* + \bB\z^* - \c & = 0~. \label{eq:kkty}
\end{align}
\fi
%$\{ \x^*, \z^*,\y^*\}$ is an optimal solution. 
The optimality conditions of~\myref{eq:badmm_x} and~\myref{eq:badmm_z} are
\begin{align}
\!\!&-\! \bA^T\{ \y_t \!+\! \rho ( - \nabla\phi  (\c \!-\! \bA\x_{t+1}) \!+\! \nabla\phi  (\bB\z_t)\} \!-\! \rho_{\x}(\nabla\varphi_{\x}(\x_{t+1}) \!-\! \nabla\varphi_{\x}(\x_{t})) \!\in\! \partial f(\x_{t+1})~,\label{eq:fgd}  \\
% \end{align}
%Setting the derivative with respect to $\z$ to 0 in~\myref{eq:badmm_z}, we have
%\begin{align}
\!\!&-\! \bB^T\{ \y_t \!+\! \rho ( \nabla\phi  (\bB\z_{t+1}) \!-\! \nabla\phi  (\c \!-\! \bA\x_{t+1})\}  \!-\! \rho_{\z}(\nabla\varphi_{\z}(\z_{t+1}) \!-\! \nabla\varphi_{\z}(\z_{t}))\! \in\! \partial g(\z_{t+1})~.\label{eq:ggd}
\end{align}
If $\bA\x_{t+1} + \bB\z_{t+1} = \c$, then $\y_{t+1} = \y_t$. Therefore, the KKT conditions in~\myref{eq:kkt} are satisfied if the following optimality conditions are satisfied:
%\myref{eq:kktx} is satisfied if $\bA\x_{t+1} + \bB\z_{t} = \c~, B_{\varphi_{\x}}(\x_{t+1},\x_{t}) = 0$ in~\myref{eq:fgd}. Similarly, \myref{eq:kktz} is satisfied if $B_{\varphi_{\z}}(\z_{t+1},\z_{t}) = 0$ in \myref{eq:ggd}. Overall, the KKT conditions~\myref{eq:kkt} are satisfied if the following optimality conditions are satisfied:
\begin{subequations}\label{eq:optcd}
\begin{align}
\!\!\!\!\!\!\!\! B_{\varphi_{\x}}(\x_{t+1},\x_{t}) &= 0~,~B_{\varphi_{\z}}(\z_{t+1},\z_{t}) = 0~, \label{eq:optcd0}\\
\!\!\!\!\! \bA\x_{t+1} + \bB\z_{t} - \c &= 0~,~ \bA\x_{t+1} + \bB\z_{t+1} - \c = 0~.\label{eq:optcd1}
\end{align}
\end{subequations}
%In generalized ADMM~\cite{deng12:admm}, if $B_{\varphi_{\x}}(\x_{t+1},\x_{t}) = \frac{1}{2}\|\x - \x_t \|_{\bG}^2$.
For the exact BADMM, $\rho_\x = \rho_\z = 0$ in~\myref{eq:badmm_x} and~\myref{eq:badmm_z}, the optimality conditions are~\myref{eq:optcd1},
\iffalse
% we have the following optimality conditions:
% \begin{align}\label{eq:optcd0}
% \bA\x_{t+1} + \bB\z_{t} - \c = 0~,~ \bA\x_{t+1} + \bB\z_{t+1} - \c = 0~,
% \end{align}
% which are a subset of conditions of~\myref{eq:optcd}. 
\fi
which is equivalent to the optimality conditions of ADMM ~\cite{boyd10}, i.e., $\bB\z_{t+1} - \bB\z_{t} = 0~,~ \bA\x_{t+1} + \bB\z_{t+1} - \c = 0$.
%\begin{align}
%\bB\z_{t+1} - \bB\z_{t} = 0~,~ \bA\x_{t+1} + \bB\z_{t+1} - \c = 0~.
%\end{align}
Define the residuals of optimality conditions~\myref{eq:optcd} at $(t+1)$ as:
\begin{align}\label{eq:residual}
\!\!\!\!\!\!\!R(t\!+\!1) \!=\! \frac{\rho_{\x}}{\rho} B_{\varphi_{\x}} \!(\x_{t+1},\!\x_t) \!+\! \frac{\rho_{\z}}{\rho} \! B_{\varphi_{\z}}\!(\z_{t+1},\!\z_t) \!+\!\! B_{\phi}(\c \!-\!\! \bA\x_{t+1}, \!\bB\z_t) \!+\! \gamma \| \bA\x_{t+1}  \!\!+\!  \bB\z_{t+1} \!\!-\! \c \|_2^2~,\!\!\!
\end{align}
where $\gamma > 0$. If $R(t+1) = 0$, the optimality conditions~\myref{eq:optcd0} and~\myref{eq:optcd1} are satisfied.
It is sufficient to show the convergence of BADMM by showing $R(t+1)$ converges to zero. 
\iffalse
We need the following lemma.
%by showing that the distance between the objective value at $t+1$ and the optimal value is bounded by some telescoping series.
\begin{lem}\label{lem:fgobj}
Let the sequence $\{\x_t, \z_t,\y_t\}$ be generated by Bregman ADMM~\myref{eq:badmm_x}-\myref{eq:badmm_y}. For any $\x^*,\z^*$ satisfying $\bA\x^* + \bB\z^* = \c$, we have
\begin{align}\label{eq:fg}
\!\!\!&f(\x_{t+1})+ g(\z_{t+1}) - (f(\x^*)+g(\z^*)) \nonumber \\
\!\!\!&\leq -\langle \y_t, \bA\x_{t+1} + \bB\z_{t+1} - \c \rangle - \rho ( B_{\phi}(\c -\bA\x_{t+1}, \bB\z_t) \nonumber \\ 
\!\!\!& \!\!+\!\!  B_{\phi}(\!\bB\z_{t+1},\! \c \!-\!\!\bA\x_{t+1}\!)\!) \!+\! \rho (B_{\phi}(\bB\z^*\!, \bB\z_t) \!-\! B_{\phi}(\bB\z^*\!, \bB\z_{t+1}\!)\!) \nonumber \\ 
\!\!\!& +\rho_{\x}(B_{\varphi_{\x}}(\x^*, \x_t) - B_{\varphi_{\x}}(\x^*, \x_{t+1}) - B_{\varphi_{\x}}(\x_{t+1},\x_t))\nonumber \\
\!\!\!& \!+\! \rho_{\z}(B_{\varphi_{\z}}\!(\z^*\!, \z_t) \!-\! B_{\varphi_{\z}}(\z^*\!, \z_{t+1}) \!-\! B_{\varphi_{\z}}(\z_{t+1},\z_t))
~.\!\!\!\!
\end{align}
\end{lem}

%\input{appen1}
%The proof of Lemma~\ref{lem:fgobj} is on Appendix~\ref{appen1}. 
Under Assumption~\ref{asm:badmm}(c), the following lemma shows that~\myref{eq:residual} is bounded by a telescoping series of $D(\w^*,\w_t) - D(\w^*,\w_{t+1})$, where $D(\w^*,\w_t)$ defines the distance from the current iterate $\w_t = (\x_t,\z_t,\y_t)$ to a KKT point $\w^* = (\x^*,\z^*,\y^*)$ as follows:
\begin{align}\label{eq:ht}
D(\w^*,\w_t) &= \frac{1}{2\tau\rho}\| \y^* \!-\! \y_{t}\|_2^2 + B_{\phi}(\bB\z^*, \bB\z_{t}) + \frac{\rho_{\x}}{\rho} B_{\varphi_{\x}}(\x^*, \x_{t}) \!+\! \frac{\rho_{\z}}{\rho} B_{\varphi_{\z}}(\z^*, \z_{t})~.
\end{align}

\begin{lem}\label{lem:RD}
Let the sequence $\{\x_t, \z_t,\y_t\}$ be generated by Bregman ADMM~\myref{eq:badmm_x}-\myref{eq:badmm_y} and $\{\x^*,\z^*,\y^*\}$ satisfy~\myref{eq:kkt}. Let the Assumption~\ref{asm:badmm} hold. $R(t+1)$ and $D(\w^*,\w_t)$ are defined in~\myref{eq:residual} and~\myref{eq:ht} respectively. Set $\tau \leq (\alpha \sigma  - 2 \gamma)\rho$, where $\sigma = \min\{1, m^{\frac{2}{p}-1}\}$ and $0 < \gamma < \frac{\alpha\sigma}{2}$. Then
\begin{align}\label{eq:case1}
& R(t+1) \leq D(\w^*,\w_t) - D(\w^*,\w_{t+1})~.
\end{align}
\end{lem}
\fi
%The proof of Lemma~\ref{lem:RD} is on Appendix~\ref{appen2}. 
The following theorem establishes the global convergence for BADMM.

\begin{thm} Let the sequence $\{\x_t, \z_t,\y_t\}$ be generated by BADMM~\myref{eq:badmm_x}-\myref{eq:badmm_y} and $\{\x^*,\z^*,\y^*\}$ satisfy~\myref{eq:kkt}. Let the Assumption~\ref{asm:badmm} hold and $\tau \leq (\alpha \sigma  - 2 \gamma)\rho$, where $\sigma = \min\{1, m^{\frac{2}{p}-1}\}$ and $0 < \gamma < \frac{\alpha\sigma}{2}$. Then $R(t+1)$ converges to zero and $\{\x_t,\z_t,\y_t\}$ converges to a KKT point $\{\x^*,\z^*,\y^*\}$ of~\myref{eq:adm_pm}.
%\begin{align}\label{eq:thm_opt}
%B_{\varphi_{\x}}(\x_{t+1},\x_t)\rightarrow 0, B_{\varphi_{\z}}(\z_{t+1},\z_t) \rightarrow 0,B_{\phi}(\c -\bA\x_{t+1}, \bB\z_t) \rightarrow 0, \| \bA\x_{t+1} + \bB\z_{t+1} - \c\|_2^2\rightarrow 0~,
%\end{align}
%implying the optimality conditions~\myref{eq:optcd} are satisfied.
\end{thm}

\begin{remark}\label{remark1}
%\allowdisplaybreaks
(a) If $0< p \leq 2$, then $\sigma = 1$ and $\tau \leq (\alpha - 2\gamma)\rho$. The case that $0 < p \leq 2$ includes two widely used Bregman divergences, i.e., Euclidean distance and KL divergence. For KL divergence in the unit simplex,  we have $\alpha = 1, p = 1$ in the Assumption~\ref{asm:badmm} (c), i.e., $KL(\u,\v) \geq \frac{1}{2}\|\u - \v\|_1^2$~\cite{Beck03}. 

(b) Since we often set $B_\phi$ to be a quadratic function ($p = 2$), the three special cases in Section 2.1 could choose step size $\tau = (\alpha - 2\gamma)\rho$.

(c) If $p > 2$, the proof requires a sufficiently small step size $\tau$, which may not be needed in practice. 
It would be interesting to see whether we can use a same $\tau = O(\rho)$ for any $p > 0$ using other proof techniques. 
\end{remark}


The following theorem establishes a $O(1/T)$ iteration complexity for the objective and residual of constraints in an ergodic sense.
%\subsection{$O(1/T)$ Convergence Rate for General Convex Functions}

\begin{thm} \label{thm:badmm_rate}
Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by BADMM~\myref{eq:badmm_x}-\myref{eq:badmm_y}. Set $\tau \leq (\alpha \sigma  - 2 \gamma)\rho$, where $\sigma = \min\{1, m^{\frac{2}{p}-1}\}$ and $0 < \gamma < \frac{\alpha\sigma}{2}$. Let $\bar{\x}_T = \frac{1}{T}\sum_{t=1}^T \x_t$, $\bar{\z}_T = \frac{1}{T}\sum_{t=1}^T \z_t$ and $\y_0 = \mathbf{0}$.  For any $(\x^*,\z^*,\y^*)$ satisfying KKT conditions~\myref{eq:kkt}, we have
%Setting $\tau = \alpha\rho$ if $0 < p \leq 2$ or $\tau = \alpha\rho m^{\frac{2}{p} - 1}$ (see $m$ in~\myref{eq:adm_pm}) if $p > 2$, then
\begin{align}
&f(\bar{\x}_{T}) + g(\bar{\z}_{T}) - (f(\x^*) + g(\z^*))
 \leq \frac{D_1}{T}~,\label{eq:fgrate1} \\
&\|\bA\bar{\x}_{T} + \bB\bar{\z}_{T} - \c \|_2^2 \leq \frac{D(\w^*,\w_0)}{\gamma T}~,\label{eq:cstrate1}
\end{align}
where $D_1 = \rho B_{\phi}(\bB\z^*, \bB\z_0)+ \rho_{\x}B_{\varphi_{\x}}(\x^*, \x_0) + \rho_{\z}B_{\varphi_{\z}}(\z^*, \z_0)$.
\end{thm}

We consider one special case of BADMM which could outperform ADMM. Assume $\bB = \bI$ and $\cX, \cZ$ are the unit simplex. Let $B_{\phi}$ be the KL divergence. 
For $\z \in \R^{n_2\times 1}$, we have
\begin{align}
B_{\phi}(\z^*, \z_0) = \sum_{i=1}^{n_2} z_i^* \ln \frac{z_i^*}{z_{i,0}} = \sum_{i=1}^{n_2} z_i^* \ln z_i^* + \ln n_2 \leq \ln n_2~.
\end{align}
Similarly, if $\rho_{\x} > 0$, by choosing $\x_0 = \e/n_2$, $B_{\varphi_\x}(\x^*, \x_0) \leq \ln n_1$.
Setting $\alpha = 1, \sigma = 1$ and $\gamma = \frac{1}{4}$ in Theorem~\ref{thm:badmm_rate} yields the following result:
\begin{cor} \label{cor:badmm_rate_KL}
Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by Bregman ADMM~\myref{eq:badmm_x},\myref{eq:badmm_z},\myref{eq:badmm_y} and $\y_0 = \mathbf{0}$. Assume $\bB = \bI$, and $\cX$ and $\cZ$ is the unit simplex. Let $B_{\phi}, B_{\varphi_\x}, B_{\varphi_\z}$ be KL divergence.
Let $\bar{\x}_T = \frac{1}{T}\sum_{t=1}^T \x_t$, $\bar{\z}_T = \frac{1}{T}\sum_{t=1}^T \z_t$. Set $\tau = \frac{3\rho}{4}$. For any $(\x^*,\z^*,\y^*)$ satisfying KKT conditions~\myref{eq:kkt}, we have
%Setting $\tau = \alpha\rho$ if $0 < p \leq 2$ or $\tau = \alpha\rho m^{\frac{2}{p} - 1}$ (see $m$ in~\myref{eq:adm_pm}) if $p > 2$, then
\begin{align}
& f(\bar{\x}_{T}) + g(\bar{\z}_{T}) - (f(\x^*) + g(\z^*)) \leq \frac{\rho\ln n_2  +  \rho_\x \ln n_1 + \rho_{\z} \ln n_2}{T}~,\label{eq:fgrate1} \\
&\|\bA\bar{\x}_{T} + \bB\bar{\z}_{T} - \c \|_2^2 \leq \frac{ \frac{2}{\tau\rho}\| \y^* \!-\! \y_{0}\|_2^2 + 4\ln n_2 + \frac{4\rho_{\x}}{\rho} \ln n_1 \!+\! \frac{4\rho_{\z}}{\rho} \ln n_2 }{ T}~,\label{eq:cstrate1}
\end{align}
\end{cor}

\begin{remark}
(a)  In~\cite{Beck03}, it shows that MDA yields a smilar $O(\ln n)$ bound where $n$ is dimensionality of the problem. If the diminishing step size of MDA is propotional to $\sqrt{\ln n}$, the bound is $O(\sqrt{\ln n})$. Therefore, MDA can outperform the gradient method by a factor $O((n/\ln n)^{1/2})$.

(b) With constant step size, BADMM outperforms ADMM by a factor $O(n/\ln n)$ in an ergodic sense.
\end{remark}

\iffalse
\begin{remark}
As pointed out in \myref{remark1}, a sufficiently small step size $\tau$ is required if $p > 2$. 
In Appendix 2, we also establish a $\sqrt{T}$ rate for BADMM when choosing a large step size. The  the assumption that $\y_t$ is bounded and Assumption~\ref{asm:badmm}.
In addition to the Assumption~\ref{asm:badmm}, we further assume $\y_t$ is bounded, 
BADMM requires choosing a large step size $\tau = O(\sqrt{T})$.
Under the assumption that $\y_t$ is bounded, $R(t+1)$ converges to zero when choosing $\rho_\x = \rho_\z = c_1\sqrt{T}, \tau = c_2\sqrt{T}, \rho = \sqrt{T}$ for some positive constants $c_1,c_2$, which is shown in Theorem 3 on Appendix 2. %~\ref{appen3}.~\ref{thm:cvg2}
Under the assumption that $\y_t$ is bounded, the objective converges at a rate of $O(1/\sqrt{T})$ when setting $\rho_\x,\rho_\z,\tau, \rho = O(\sqrt{T})$, 
which is established in Theorem 4 in Appendix 2. %~\ref{appen3}. ~\ref{thm:badmm_rate2} 
\end{remark}
\fi
%In (b), it does not require a sufficiently small $\tau$ but is based on the assumption that $\y_t$ is bounded. In addition, (b) introduces an additional error term to the telescoping series in~\myref{eq:case2}, which requires large values of $\rho,\tau$ to guarantee the cumulative error does not increase rapidly over $t$.


